POV: Prompt-Oriented View-Agnostic Learning for Egocentric Hand-Object Interaction in the Multi-View World

We humans are good at translating third-person observations of hand-object interactions (HOI) into an egocentric view. However, current methods struggle to replicate this ability of view adaptation from third-person to first-person. Although some approaches attempt to learn view-agnostic representation from large-scale video datasets, they ignore the relationships among multiple third-person views. To this end, we propose a Prompt-Oriented View-agnostic learning (POV) framework in this paper, which enables this view adaptation with few egocentric videos. Specifically, We introduce interactive masking prompts at the frame level to capture fine-grained action information, and view-aware prompts at the token level to learn view-agnostic representation. To verify our method, we establish two benchmarks for transferring from multiple third-person views to the egocentric view. Our extensive experiments on these benchmarks demonstrate the efficiency and effectiveness of our POV framework and prompt tuning techniques in terms of view adaptation and view generalization. Our code is available at \url{https://github.com/xuboshen/pov_acmmm2023}.

==> tables/abl_data_augmentation.tex <==
\begin{table}[t]
% \centering
\caption{Ablation study of data augmentation technique on H2O.}
\scalebox{0.9}{
\begin{tabular}{c|ccc|ccc}
\toprule
&\multicolumn{3}{c}{Assembly101} &
\multicolumn{3}{c}{H2O}\\
\midrule
\multirow{1}{*}{type} & 
verb & object & action &verb & object &action \\
\midrule
% Random &RGB&MViT& 12.65 & 41.89 & 5.74 & 25.91 & 3.74 & 10.97 & 35.304 & 71.819\\
none & - & - & - \\
horizontal clip & - & - & - \\
multi-crop & - & - & - \\
color jitter & - & - & - \\
\bottomrule
\end{tabular}
}
\label{sotas_on_assembly101}
\end{table}

==> tables/dataset.tex <==
% 主实验结果
% Comparison of important elements
\begin{table*}[bht]
\caption{\textcolor{red}{Appendix, captioning: egocentric, scenario explanation, } Video domain adaptation benchmarks descriptions. H2O and Assembly101 are our proposed version in our task. Labeled source split and unlabeled target split are used for training, while test split is used for testing. The target split and test split has no overlapping. For multi-source datasets, we choose one domain as target domain and the rest as source domain.}
% \resizebox{\linewidth}{!}{
\begin{tabular}{ccccccc}
\toprule
\multicolumn{1}{c}{dataset} & 
\multicolumn{1}{c}{scenario} &
\multicolumn{1}{c}{fine-grained} &
\multicolumn{1}{c}{multi-source} &
\multicolumn{1}{c}{\#source/target/test}& 
\multicolumn{1}{c}{domain } &
\multicolumn{1}{c}{\#category}\\
\midrule
\midrule
% Random &RGB&MViT& 12.65 & 41.89 & 5.74 & 25.91 & 3.74 & 10.97 & 35.304 & 71.819\\
ActorShift\cite{xu2021dailyda} & sports & × & × & 1305/35/165 & species & 7\\
CharadesEgo\cite{} & daily &\checkmark\kern-1.1ex\raisebox{.7ex}{\rotatebox[origin=c]{125}{--}} & × & 3083/3083/825 & viewpoint & 8\\
Epic-kitchens\cite{} & kitchen & $\checkmark$ & × & 7935/7935/2159 & scenery  & 8\\
% dailyda take 2A as example
Daily-DA\cite{} & daily & × & $\checkmark$ & 13,516/2775/1288& scenery  & 8\\
% to ucf101
TSU~\cite{} & daily & × & $\checkmark$ & - & viewpoint  & 19\\
Sports-DA\cite{} & sports & × & $\checkmark$ & 33857/2144/850 & scenery  & 23\\
\hline
H2O\cite{}& daily & $\checkmark$ & $\checkmark$ & 2764/180/511 & viewpoint   & 36\\
% 691*4
Assembly101\cite{}& industry & $\checkmark$ & $\checkmark$ &  134104/10388/10388& viewpoint   &142\\
% 33526$\times$4
\bottomrule
\end{tabular}
% }
\label{tablea}
\end{table*}
